Stable Diffusion For Aerial Object Detection

Aerial object detection is a challenging task, in which one major obstacle lies in the limitations of large-scale data collection and the long-tail distribution of certain classes. Synthetic data offers a promising solution, especially with recent advances in diffusion-based methods like stable diffusion (SD). However, the direct application of diffusion methods to aerial domains poses unique challenges: stable diffusion's optimization for rich ground-level semantics doesn't align with the sparse nature of aerial objects, and the extraction of post-synthesis object coordinates remains problematic. To address these challenges, we introduce a synthetic data augmentation framework tailored for aerial images. It encompasses sparse-to-dense region of interest (ROI) extraction to bridge the semantic gap, fine-tuning the diffusion model with low-rank adaptation (LORA) to circumvent exhaustive retraining, and finally, a Copy-Paste method to compose synthesized objects with backgrounds, providing a nuanced approach to aerial object detection through synthetic data.

==> sec2_related.tex <==

\section{Related Works}
\label{gen_inst}
Several works have explored the effectivness of data augmentation on general object detection dataset like COCO. Ghiasi et.al \cite{ghiasi2021simple} explores the effectiveness of the Copy-Paste augmentation method, where objects are randomly pasted onto images, and reveals that this simple approach yields substantial performance gains when combined with strong baselines. Moreover, it demonstrates that Copy-Paste augmentation is complementary to semi-supervised methods that use pseudo labeling.
Zhao et.al \cite{zhao2023xpaste} Futher explores the scalibility of Copy-Paste augmentation,  by harnessing the capabilities of zero-shot recognition models like CLIP and text2image models such as StableDiffusion. They demonstrate that using text2image models to generate images or zero-shot recognition models to filter noisy crawled images for various object categories is a viable approach to scale up Copy-Paste augmentation.

Our approach is inspired by the above methods. In our case, the long-tail classes don't have good representations generated with zero-shot text2image model, thus, we instead use a simple and straight forward way to add text promopt and finetune StableDiffusion (SD) model to generate similar looking images with good amount of variety. Considering the sparse object presence and their tiny sizes, we do sparse-dense cropping on the original detection dataset, finetune SD on the crops, then inference SD to generate various instances for each class, finally we Copy-Paste the generated images onto background from original detection dataset to compose synthetic data. 
